In-Context Learning May Not Elicit Trustworthy Reasoning: A-Not-B Errors in Pretrained Language Models

Recent advancements in artificial intelligence have led to the creation of highly capable large language models (LLMs) that can perform tasks in a human-like manner. However, LLMs exhibit only infant-level cognitive abilities in certain areas. One such area is the A-Not-B error, a phenomenon seen in infants where they repeat a previously rewarded behavior despite well-observed changed conditions. This highlights their lack of inhibitory control -- the ability to stop a habitual or impulsive response. In our work, we design a text-based multi-choice QA scenario similar to the A-Not-B experimental settings to systematically test the inhibitory control abilities of LLMs. We found that state-of-the-art LLMs (like Llama3-8b) perform consistently well with in-context learning (ICL) but make errors and show a significant drop of as many as 83.3% in reasoning tasks when the context changes trivially. This suggests that LLMs only have inhibitory control abilities on par with human infants in this regard, often failing to suppress the previously established response pattern during ICL.

==> header.tex <==
% \documentclass[11pt]{article}

% \usepackage[preprint]{acl}
% % \usepackage[final]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{booktabs}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{microtype}
% \usepackage{inconsolata}
% \usepackage{graphicx}


% % Recommended, but optional, packages for figures and better typesetting:
% \usepackage{microtype}
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables

% \usepackage{xcolor}
% \usepackage{xspace}
% \usepackage{tcolorbox}

% \definecolor{lightBlue}{rgb}{0.78, 0.85, 1.0}
% \definecolor{lightRed}{rgb}{1.0, 0.85, 0.85}
% \newtcbox{\bluebox}{on line, box align=base, colback=lightBlue,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\redbox}{on line, box align=base, colback=lightRed,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newcommand{\uarr}{$\uparrow$}
% \newcommand{\darr}{$\downarrow$}

% \usepackage{hyperref}
% \usepackage{multicol}
% \usepackage{multirow}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% % For theorems and such
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage{amsthm}

% % if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % color
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{colortbl}
% \usepackage{pgf} % for calculating the values for gradient
% \usepackage{xcolor} % enables the use of cellcolor
% \usepackage{graphicx}
% \usepackage{booktabs} % for better table formatting (optional)

% \definecolor{lightOliveGreen}{rgb}{0.75, 0.85, 0.65} % Light Olive Green (adjust as necessary)
% \definecolor{lightTomatoRed}{rgb}{1.0, 0.7, 0.6}     % Light Tomato Red (adjust as necessary)

% \newtcbox{\greenbox}{on line, box align=base, colback=lightOliveGreen, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\tomatobox}{on line, box align=base, colback=lightTomatoRed, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}





% % Color set related to your provided highlight.sty
% \definecolor{high}{HTML}{6B8E23}  % The color for increases (Olive Green)
% \definecolor{lowgreen}{HTML}{F0F8E7}  % A very light green for the lower end of the gradient
% \definecolor{redhigh}{HTML}{FF6347} % The color for decreases (Red, Tomato)
% \definecolor{lowred}{HTML}{FFE6E6}  % A very light red for the lower end of the gradient
% \newcommand{\opacity}{50}         % Opacity set to 50 (higher opacity, but you can reduce further if needed)

% % Gradient function for increases (Olive Green)
% \newcommand*{\minvaldiffa}{0}% define the minimum value on your data set
% \newcommand*{\maxvaldiffa}{50}% define the maximum value in your data set!
% \newcommand{\gcb}[1]{
%     \pgfmathparse{min(#1,\maxvaldiffa)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{max(\clipval,\minvaldiffa)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{int(round(100*(\clipval/(\maxvaldiffa-\minvaldiffa))-(\minvaldiffa*(100/(\maxvaldiffa-\minvaldiffa)))))}%
%     \xdef\tempa{\pgfmathresult}%
%     \cellcolor{high!\tempa!lowgreen!\opacity}%
%     $#1$%
% }

% % Gradient function for decreases (Red)
% \newcommand*{\minvaldiffb}{0}% define the minimum value on your data set
% \newcommand*{\maxvaldiffb}{50}% define the maximum value in your data set!
% \newcommand{\gca}[1]{
%     \pgfmathparse{min(#1,\maxvaldiffb)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{max(\clipval,\minvaldiffb)}%
%     \xdef\clipval{\pgfmathresult}%
%     \pgfmathparse{int(round(100*(\clipval/(\maxvaldiffb-\minvaldiffb))-(\minvaldiffb*(100/(\maxvaldiffb-\minvaldiffb)))))}%
%     \xdef\tempa{\pgfmathresult}%
%     \cellcolor{redhigh!\tempa!lowred!\opacity}%
%     $#1$%
% }


% \title{In-Context Learning May Not Elicit Trustworthy Reasoning: A-Not-B Errors in Pretrained Language Models}

% \author{%
%     Pengrui Han\thanks{Equal contribution.}\thanks{Work done as intern.}$^{\,1,3}$, Peiyang Song\footnotemark[1]$^{\,2}$, Haofei Yu$^{\,3}$, Jiaxuan You$^{\,3}$ \\
%     $^1$Carleton College, ~$^2$California Institute of Technology\\
%     $^3$University of Illinois Urbana-Champaign\\
%     \texttt{barryhan@carleton.edu}, \texttt{psong@caltech.edu} \\
% }

